Generative Framework for Personalized Persuasion: Inferring Causal, Counterfactual, and Latent Knowledge

We hypothesize that optimal system responses emerge from adaptive strategies grounded in causal and counterfactual knowledge. Counterfactual inference allows us to create hypothetical scenarios to examine the effects of alternative system responses. We enhance this process through causal discovery, which identifies the strategies informed by the underlying causal structure that govern system behaviors. Moreover, we consider the psychological constructs and unobservable noises that might be influencing user-system interactions as latent factors. We show that these factors can be effectively estimated. We employ causal discovery to identify strategy-level causal relationships among user and system utterances, guiding the generation of personalized counterfactual dialogues. We model the user utterance strategies as causal factors, enabling system strategies to be treated as counterfactual actions. Furthermore, we optimize policies for selecting system responses based on counterfactual data. Our results using a real-world dataset on social good demonstrate significant improvements in persuasive system outcomes, with increased cumulative rewards validating the efficacy of causal discovery in guiding personalized counterfactual inference and optimizing dialogue policies for a persuasive dialogue system.

==> 8-_Not_Submitted__Conclusion.tex <==
\section{Conclusion}
In this paper, we addressed the limitations of current persuasive conversation systems, particularly their struggle to dynamically adapt to personalized user traits and understand the causal relationships between user responses and outcomes. We proposed a novel approach that integrates causal discovery (via GRaSP) with personalized counterfactual reasoning to optimize persuasion outcomes (by augmenting BiCoGAN and KQR with our TP3M). Our approach generates more principled and grounded counterfactual actions based on underlying causal structures at the dialogue strategy level.

Our experimental results show that this approach significantly enhances cumulative rewards (representing the actual donations) in dialogue interactions compared to baseline methods on the PersuasionForGood dataset. These findings demonstrate the power of combining causal discovery-driven counterfactual reasoning with policy learning to create adaptive, personalized, and highly effective persuasive systems.
% Our results show that this approach enhances the persuasive system's ability to generate personalized counterfactual utterances. This approach combined with optimal policy learning (via D3QN) outperforms our baseline methods using the PersuasionForGood dataset. This demonstrates that our method not only improves cumulative rewards but also increased the cumulative actual donations over the dialogues contrast to the actual donations in the dataset. All of these confirm the effectiveness of leveraging causal discovery and personalized counterfactual reasoning in optimizing persuasive interactions. 
In the future, we plan to further analyze the causal discovery results, and make the causal discovery task even more principled when necessary, to further enhance the creation of counterfactual data that could empower the system with more efficacious persuasive responses.

==> 8-_Previous__Discussion.tex <==
\section{Discussion}
PTs often need personalized data to effectively tailor their messages, suggestions, or interventions. Without sufficient data on target users, it is difficult to design systems that account for individual differences in psychological constructs like personality traits. Furthermore, the fact that persuasion relies heavily on the context in which a person is situated, limited data makes it harder to understand contextual factors that can arise as latent noises. 
%Furthermore, persuasive techniques and methods embedded in persuasive technologies are carefully crafted based on established theories (e.g., Cialdini's famous principles of persuasion~\cite{Cialdini2001, Cialdini2006}) or frameworks (the well-known Persuasive Systems Design~\cite{OinasKukkonen2009}) of how people are influenced. 
%Thus, we reckon that there should be enough space for PTs to navigate in dynamically changing contexts to be effective.

Our work is data-centric, and extends beyond what is observable in the data. We address data scarcity through data augmentation by creating alternative reality data points that are still identifiable from the ground truth. 
%
From a technical standpoint, something that is typically a concern with counterfactuals is whether they will be in-distribution. However, we alleviated this issue by leveraging causal relations that were inferred from the observed data to generate the counterfactuals. 
%
Another possible issue is that our evaluation is primarily done with a specific dataset, i.e., P4G. Although we detailed our good results that delve into the learned structural causal models as well as the success measures, indeed, one can argue that with one dataset, the generalization ability of our framework in other types of persuasion tasks has not been fully explored. While this is a fair point, we reckon that our study can lay the groundwork for developing a generative AI of this kind: enable a system to simulate ``what-if'' scenarios, broadening the dataset with hypothetical yet realistic interactions, while minimizing the need for extensive data collection especially when direct experimentation is infeasible. 
%
To adapt our framework to suit, inter alia, recommendation, health intervention, and negotiation tasks is for us an exciting prospect. But our goal for now is to achieve a good foundation before progressing to other complex tasks.
Furthermore, although P4G was conceived on the idea of altering users’ opinions and actions on donating, in a broader sense, the aim for this  dataset is for it to facilitate the development of intelligent persuasive conversational agents~\cite{Wang2019}.

Additionally, estimating the presence and influence of latent factors also plays a pivotal role. Our findings show that estimating latent influences, especially when explicitly done, leads to more robust outcomes. By capitalizing on latent factors, systems can pragmatically improve performance without being overly reliant on abstract principles. 

%Estimation of latent influences, generating high-quality augmented data, and achieving adaptive personalization are critical challenges in real-world PTs. Our personalized causality-based generative persuasion framework addresses these challenges by leveraging causal knowledge for dynamic user-adaptation. 
% The results from testing our personalized causality-based generative persuasion framework using an actual dataset for promoting social good highlight several important insights. First, causal knowledge significantly enhances counterfactual inference, enabling the creation of realistic, previously unobserved scenarios from limited datasets.  By embedding this causal understanding into our models, we demonstrate how causal relations that enhance the generation of diverse and effective system actions, evidenced by the improved persuasion outcomes.



\section{Shaping Ethics in Generative AI}

Our work underscores the ethical and practical implications of generative AI in persuasive technology (GenAI-PT). This study demonstrates that when applied responsibly to socially beneficial purposes, GenAI-PT can be a force to drive positive change. The potential for harm, such as manipulative persuasions, is mitigated in our study by focusing on social good, as demonstrated through increased charitable donations from our counterfactual datasets. Furthermore, our method is unbiased as it does not overly rely on personality stereotypes, some of which may not be true, hence, can be harmful. Instead, it dynamically fine-tunes its personality trait estimates based on the utterances in the ensuing dialogue. 

While theory-centric approaches often risk homogenization and overlook diverse user contexts, our framework ensures adaptability to personal and contextual scenarios by accounting for latent influences. Furthermore, by ensuring that the system adapts to evolving user states and aligns its strategies with their shifting needs, we prioritize towards long-term relevance and user well-being. Future enhancements of our framework could enable continual learning and self-improvement to foster enduring, trust-based relationships between persuasive agents and their users (e.g., in~\cite{Legaspi2021}).

\begin{comment}

Estimation of influencing latent noises, generation of high-quality augmented data, and achieving adaptive personalization are significant challenges in real-world applications including persuasive technologies. Our personalized causation-based generative persuasion architecture is an attempt to come closer to overcoming these challenges, and by testing this architecture using an actual dataset to persuade for social good, our results suggest the following:
\begin{itemize}
    \item \textit{Causal knowledge enhances counterfactual inference of possible alternative reality.} This is significantly demonstrated by our results. By commencing with a causal structure in mind (e.g., a hypothesis-driven research), it is only reasonable to extract causal conclusions when prior knowledge ascertains that the relationships are by all means causal~\cite{Runge2019}. Yet, in situations where conducting real experiments is not possible or knowledge about the underlying causations are nowhere to be found, discovering the causal structure from data becomes essential. The desirable aspect here is the ability to recover temporal causal relationships from limited non-expert datasets that allow the creation of unobserved yet realistic scenarios.     
    \item \textit{Estimating both recoverable and unidentifiable latent noises leads to better outcomes.} We expected initially that KQR, by not estimating the latent noises, would lead to better persuasion outcomes (optimized most of the cumulative rewards) than BiCoGAN which estimates the noises. This would indeed be cutting edge if such a method does not need to estimate any latent psychological or environmental latent factors. Nonetheless, the results from KQR with no causal discovery are still at par with the ground truth cumulative rewards, and better yet, its persuasion outcomes dramatically increase with causal knowledge. What the variants of BiCoGAN demonstrated is the benefit of independently estimating for recoverable and unidentifiable noises. It can also be said that capitalizing on recoverable noises is pragmatic, i.e., why not leverage practicality over abstract principles when by predicting what is recoverable would reveal more information on the influence of noise on the system efficacy.
   \item \textit{Dynamic adaptation is possible with the recovered latent personality dimensions.} By continuously inferring, tracking, and adapting to the user's hidden OCEAN states, an agent can generate persuasive utterances that are aligned with the evolving trait-based perceptions of the user. This dynamic personalization enhances the effectiveness of the dialogue as it captures nuanced changes in the user's mental state over time.     
    \item \textit{Counterfactual inference improves the persuasive dialogue outcomes.} By examining \textit{what-if} scenarios and adjusting persuasive strategies based on these hypothetical situations, the chances of the persuasive agent successfully achieving its desired persuasion goals increase. Indeed, this is evidenced by the improved cumulative rewards in our results. A key feature here is the ability to derive sequential cause-and-effect relationships between utterance strategies from a limited non-expert dataset, enabling the emergence of realistic yet previously unobserved scenarios. This significantly minimizes the need for large-scale data collection, and by simulating different state-action pairs through hypothetical actions, our approach enhances the training dataset with a wide variety of diverse dialogue utterances.
    \item \textit{Our work has implication for future persuasive systems.} This study demonstrates that persuasive dialogue systems can move beyond static models and pre-defined strategies. By incorporating causal reasoning and dynamically adapting to user states, systems can deliver more flexible, context-aware, and personalized interactions. This has broad implications for applications in marketing, health communication, and social good initiatives (e.g., see~\cite{Furumai2024PersuaBot}).
\end{itemize}

Here are some of what we propound are the ethical, as well as practical and social, implications of our study:
\vspace{-\topsep}
\begin{itemize}
    \item Data-centric persuasive systems would often rely on user profiles and preferences, which may inadvertently lead to homogenized solutions that fail to reflect diverse cultural, social, or personal contexts. Our study, by being cognizant of latent noises, recoverable or unidentifiable, aims to ensure that a persuasive system can adapt to diverse users.
    \item Persuasive systems, by nature, attempt to influence user behavior, which can very well lead to harm, such as manipulation - especially if users are unaware of how their behavior is being influenced. This is certainly possible with our approach if the system is given a maleficent or malicious persuasive goal. By using a dataset on social good and producing persuasion outcomes that improve for social good, what our study aims to demonstrate is that our architecture can be a force for positive change when applied responsibly for socially good purposes. This is evidenced by the increased cumulative donation amount as shown by our results.
    \item A persuasive system that does not account for the user’s evolving context might push for behavior that is not in the user's best interest, especially if it is ignoring their shifting needs or values. Thus, we designed our causal discovery in such a way that the user takes the lead and the persuasive system adjusts its strategies based on the user's strategies, without compromising or abandoning its persuasion goal.
    \item For persuasive systems to work in the long term, they need flexibility to understand and respond to the fluid nature of human behavior and the contexts in which it occurs. Without this adaptability, the system risks becoming irrelevant, intrusive, or even harmful. This is what our study aims to achieve, and perhaps, what we can do next is to enable our architecture to open itself up for continual learning and self-improvement for its persuasive agent to build long-term relationships with user persuadees.
\end{itemize}

\end{comment}

%We also encourage authors to discuss potential ethical considerations of their work; aspects pertaining to current societal issues; diversity, inclusion, and equality; and other topics under the broad responsible AI topic. We encourage authors to consider practical and societal implications of their work (as well as its shortcomings) throughout their projects and to include a reflection on those implications in their papers, in particular how the proposed methods and insights could be applied and deployed in a realistic setting and how they can improve people’s lives in the real world.
% \textcolor{red}{\textbf{
% Zeng-san, please share here your insights and take-away based on the results. Please avoid repeating what has already been said in the above sections and should not also repeat what is in the Conclusion. 
% The key thing here is for us to state what we want the readers and reviewers to bring home as deep and insightful knowledge.
% //Ex: Implication to PT in general
% }}
